Multimodal Large Language Models as Image Classifiers

Multimodal Large Language Model (MLLM) classification performance depends critically on evaluation protocol and ground truth quality. Studies comparing MLLMs with supervised and Vision-Language Models (VLMs) report conflicting conclusions, and we show these conflicts stem from protocols that either inflate or underestimate performance. Across the most common evaluation protocols, we identify and fix key issues: model outputs that fall outside the provided class list and are discarded, inflated results from weak multiple-choice distractors, and open-world setting that underperforms only due to poor output mapping. We additionally quantify the impact of commonly overlooked design choices - batch size, image ordering, and text encoder selection - showing they substantially affect accuracy. Evaluating on ReGT, our multilabel reannotation of 625 ImageNet-1k classes, reveals that MLLMs benefit most from corrected labels (up to +10.8%), substantially narrowing the perceived gap with supervised models. Much of the reported MLLM underperformance on classification is thus an artifact of noisy ground truth and flawed evaluation protocol rather than genuine model deficiency. Models less reliant on supervised training signals prove most sensitive to annotation quality. Finally, we show that MLLMs can assist human annotators: in a controlled case study, annotators confirmed or integrated MLLM predictions in approximately 50% of difficult cases, demonstrating their potential for large-scale dataset curation. This work is part of the Aiming for Perfect ImageNet-1k project, see https://klarajanouskova.github.io/ImageNet/.

==> fig/tasks_compare.tex <==
\begin{figure}[ht]
    \centering
    \resizebox{0.7\columnwidth}{!}{%
        \includegraphics{fig/chatgpt_vs_qwen_plot.png}%
    }
    \caption{\ac{mllm} accuracy on ReGT labels categorized by tasks: Closed-set (CW), Open World (OW) and Closed World with out-of-prompt (OOP) predictions mapping (CW+). CW+ is designed to outperform CW, and it does. CW performs better than OW for \cgpt{}, while the opposite is true for \qwen{}. The latter result does not align with previous work, where CW setups typically perform much better than OW. Moreover, the accuracy gap between \qwen{} and \cgpt{} is twice as small in the OW setup as in the CW setup.}
    \label{fig:compare_tasks}
\end{figure}

==> tables/mcq_small.tex <==
\begin{table}[ht]
\small
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lc}
\toprule
Distractors & $\mathrm{A_{625}}$ (ReGT) \\
\midrule
ImGT + ReGT + random        & 94.89 \textsuperscript{\scriptsize$\pm$0.13} \\
ReGT + conf(ReGT)           & 84.26 \textsuperscript{\scriptsize$\pm$0.37} \\
ImGT + 999 (std. Closed World)& 81.32 \textsuperscript{\scriptsize$\pm$0.18} \\
\bottomrule
\end{tabular}
\caption{ReGT classification accuracy (A$_{625}$) for ChatGPT in the 4-way multiple-choice task under different distractor setups.}
\label{tab:mc_chatgpt_subset}
\end{table}

